Neural Program Repair by Jointly Learning to Localize and Repair

Due to its potential to improve programmer productivity and software quality, automated program repair has been an active topic of research. Newer techniques harness neural networks to learn directly from examples of buggy programs and their fixes. In this work, we consider a recently identified class of bugs called variable-misuse bugs. The state-of-the-art solution for variable misuse enumerates potential fixes for all possible bug locations in a program, before selecting the best prediction. We show that it is beneficial to train a model that jointly and directly localizes and repairs variable-misuse bugs. We present multi-headed pointer networks for this purpose, with one head each for localization and repair. The experimental results show that the joint model significantly outperforms an enumerative solution that uses a pointer based model for repair alone.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#
NAME=main
PACKAGE=acmart

SAMPLES = \
	main.tex

PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

main.pdf: main.tex

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM) *.log *.aux $(NAME).pdf \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> abstract-long.tex <==
\begin{abstract}
Machine-learning approaches to repairing buggy code are improving rapidly, as large source-code corpora become available, and a combination of old and new techniques are applied to modeling software. Machine-learning models that can predict a repair to a buggy program location have been achieving high accuracies even on ``real'' programming languages and code; in this paper we focus on the \emph{variable misuse} repair problem, state-of-the-art repair accuracies surpass 80\%. Such repair models have been used in an \emph{enumerative} fashion to both find and fix bugs: since the location of the bug to fix is unknown, a repair prediction is applied to every possible bug location, and those predictions that yield an answer that disagrees with the candidate program with high-enough confidence are flagged as likely bugs and repairs.  We recognize that this enumerative approach is problematic: in the presence of real bugs, the repair model is asked to predict from the wrong distribution. Instead, we propose a new model architecture, based on multi-head pointer networks, to simultaneously find the buggy location and to repair the found bug. Since the two related tasks are trained on the right distributions, their performance when applied in practice is superior to enumeratively applied repair models. We demonstrate the trouble with the existing approach, demonstrate that our joint-task model performs better, and we compare to state-of-the-art results on variable misuse, showing evidence that such joint models for localization and repair can achieve high accuracy while requiring less detailed input data and features, with better scalability, and at significantly lower training cost.
\end{abstract}


==> figures/iterative.tex <==
\centering
\begin{minipage}{\textwidth}
\begin{lstlisting}[frame=tlbr,basicstyle=\small\ttfamily]
def mul_add(a, b, c):
  return (*\hlplacehld{c}{1}*) * ((*\hlplacehld{a}{2}*) + (*\hlplacehld{b}{3}*))
\end{lstlisting}
\end{minipage}
\begin{minipage}{\textwidth}\small
\hlreflarge{1}:
\id{a}:10\%, \id{b}:10\%, \underline{\id{c}}:80\% \\
\hlreflarge{2}:
\underline{\id{a}}:75\%, \id{b}:15\%, \id{c}:10\% \\
\hlreflarge{3}:
\id{a}:5\%, \underline{\id{b}}:90\%, \id{c}:5\% \\
\end{minipage}


==> figures/iterative_error.tex <==
\centering
\begin{minipage}{\textwidth}
\begin{lstlisting}[frame=tlbr,basicstyle=\small\ttfamily]
def mul_add(a, b, c):
  return (*\hlplacehld{c}{1}*) * (c * b)
\end{lstlisting}
\end{minipage}
\begin{minipage}{\textwidth}\small
\hlreflarge{1}:
\id{a}:60\%, \id{b}:10\%, \underline{\id{c}}:30\% \\
\end{minipage}


==> motivation.tex <==
\section{Motivation}

In the enumerative approach, for each variable usage in the program separate prediction is made.
Given a program, a separate problem is constructed for each variable usage, and model is trained to predict the correct variable to fill the spot.
If prediction confidence is above a threshold value than the prediction is shown to a user.
An illustration of this approach is shown in Figure~\ref{iterexample}.

%% The \iterativeApproachName approach iteratively tries each variable location in the program to make a prediction. Given a Python program, it constructs a slot for each variable usage and uses the Graph embedding model to make the repair prediction. It then uses a threshold value to decide whether to show the prediction back to the user. An example prediction for the predictive model is shown in Figure~\ref{iterexample}.

\begin{figure}
  \centering
  \includegraphics{figures/iterative_draw}
  \caption{Iterative approach. Original program is shown on the left.
    For each variable usage separate problem is created (shown on the
    right), with a hole (green rectangle) in place of the
    variable. Model is trained to predict the correct usage.}
  \label{iterexample}
\end{figure}

%% \begin{figure}[t]
%%   \include{figures/iterative}
%%   \caption{Iterative approach. For each variable in a program, a copy
%%     of the program with a hole in place of the variable is created,
%%     and model tries to predict a correct variable for the hole. Each
%%     line below the program demonstrates models predictions for a given
%%     hole---e.g., for the hole 1, model predicts variable c with 80\%
%%     confidence.}
%%   \label{iterexample2}
%% \end{figure}


%% The \iterativeApproachName model is inefficient since it makes a prediction for each variable usage, even if the variable used is correct.
%% Assuming that most of the variable in program are correct, model makes many unnecessary predictions.
%% Moreover, model declares error only if a prediction confidence is above the threshold---setting a threshold value is not straightforward.

The \iterativeApproachName model, in addition to being inefficient and needing several threshold values, suffers from a key technical problem of the mismatch between the training and test data distribution.
\todom{MV: What do we mean by inefficient? Is it that we have to make a prediction for each variable usage, instead of making prediction only for incorrect variables? Should we ellaborate this?}
Concretely, the training is done assuming other parts of the code are correct, while only the slot variable is potentially incorrect.
However, at test time, there may be variable misuses in other parts of the code.
%% Concretely, the training of the program models is performed assuming other parts of the code are mostly correct and only the slot variable is potentially incorrect, whereas at test time, the iterative approach performs predictions for slots in the programs with additional incorrect variable usages.
An example of this mismatch is shown in Figure~\ref{datamismatch}. As we later show experimentally, this data distribution mismatch can lead to significant drop in prediction accuracy for repairs -- more than 10\% when small modifications/errors are introduced near the slot locations.

\begin{figure}
  \centering
  \includegraphics{figures/iterative_error_draw}
  \caption{Iterative approach mismatch between training and test. The
    model predicts correctly the variable for the hole (green
    rectangle) when rest of the code is correct (left). However, when
    an additional error exists (variable $c$ highlighed red) model
    mispredicts.}
  \label{datamismatch}
\end{figure}

%% \begin{figure}[t]
%%   \include{figures/iterative_error}
%%   \caption{Iterative approach with mutliple errors in program. }
%%   \label{iterexample_error}
%% \end{figure}

In contrast, our approach uses pointer network models to perform joint prediction of both the error location and the repair.
It exploits the property of the \textsc{VarMisuse} problem that both a variable misuse bug and the repair variable exist in the original program.
An overview of our approach is shown in Figure~\ref{modeloverview}.
The model first uses an LSTM based sequence encoder for the input program tokens, which are then used to train two pointers -- the first pointer corresponds to the error location of the variable misuse, and the second pointer corresponds to the repair candidate.
The pointers correspond to distributions over program tokens.
The model is trained end-to-end on a training dataset comprising of large number of programs (assumed to be mostly correct) consisting of an optional variable misuse bug.
\todom{MV: Do we try with multiple variable misuse bugs? Should we elaborate why we only choose one}
For programs where such a bug is introduced, we capture the location of the bug and the location of the original variable as the labels for the two pointers.
For programs where no variable misuse bug was introduced, the location pointer is trained to point to a special token location in the program (the first index for our experiments).

\begin{figure}
  \centering
  \includegraphics{figures/localize_and_fix_draw}
  \caption{Our approach. Model first predicts location of the error, and than predicts a variable to repair the error.}
  \label{modeloverview}
\end{figure}


==> tables/pytest_transfer.tex <==
\begin{tabular}{l|l|rr}
\toprule
\TNC{1}{\HighlightCell{Model}} \vline & \TNC{1}{\HighlightCell{Dataset}} \vline & \TNC{2}{\HighlightCell{Test Accuracy}} \\
\TNC{1}{} \vline & \TNC{1}{} \vline & \TNC{1}{Filtered} & \TNC{1}{All} \\
\midrule
lstm & original & 87.04\% & 51.01\% \\
lstm & canonicalized & 82.59\% & 82.52\% \\
lstm\_eval\_masking & original & 89.06\% & 52.21\% \\
lstm\_eval\_masking & canonicalized & 82.70\% & 82.63\% \\
lstm\_masking & original & 85.49\% & 53.58\% \\
lstm\_masking & canonicalized & 82.86\% & 82.80\% \\
pointer & original & 81.91\% & 79.34\% \\
pointer & canonicalized & 85.17\% & 80.36\% \\
\bottomrule
\end{tabular}


==> tables/statistics.tex <==
\begin{tabular}{l|l|rr}
\toprule
\TNC{1}{\HighlightCell{Model}} \vline & \TNC{1}{\HighlightCell{Dataset}} \vline & \TNC{2}{\HighlightCell{Test Accuracy}} \\
\TNC{1}{} \vline & \TNC{1}{} \vline & \TNC{1}{Filtered} & \TNC{1}{All} \\
\midrule
lstm & original & \UseMacro{lstm_eth_full_dataset_test_accuracy}\% & \UseMacro{lstm_eth_full_dataset_test_accuracy_all_examples}\% \\
lstm & canonicalized & \UseMacro{lstm_eth_canonicalized_full_dataset_test_accuracy}\% & \UseMacro{lstm_eth_canonicalized_full_dataset_test_accuracy_all_examples}\% \\
lstm\_eval\_masking & original & 86.78\% & 60.21\% \\
lstm\_eval\_masking & canonicalized & 81.74\% & 81.65\% \\
lstm\_masking & original & \UseMacro{lstm_masking_eth_full_dataset_test_accuracy}\% & \UseMacro{lstm_masking_eth_full_dataset_test_accuracy_all_examples}\% \\
lstm\_masking & canonicalized & \UseMacro{lstm_masking_eth_canonicalized_full_dataset_test_accuracy}\% & \UseMacro{lstm_masking_eth_canonicalized_full_dataset_test_accuracy_all_examples}\% \\
pointer & original & \UseMacro{pointer_eth_full_dataset_test_accuracy}\% & \UseMacro{pointer_eth_full_dataset_test_accuracy_all_examples}\% \\
pointer & canonicalized & \UseMacro{pointer_eth_canonicalized_full_dataset_test_accuracy}\% & \UseMacro{pointer_eth_canonicalized_full_dataset_test_accuracy_all_examples}\% \\
\bottomrule
\end{tabular}

